Retrofitting Contextualized Word Embeddings with Paraphrases

Contextualized word embedding models, such as ELMo, generate meaningful representations of words and their context. These models have been shown to have a great impact on downstream applications. However, in many cases, the contextualized embedding of a word changes drastically when the context is paraphrased. As a result, the downstream model is not robust to paraphrasing and other linguistic variations. To enhance the stability of contextualized word embedding models, we propose an approach to retrofitting contextualized embedding models with paraphrase contexts. Our method learns an orthogonal transformation on the input space, which seeks to minimize the variance of word representations on paraphrased contexts. Experiments show that the retrofitted model significantly outperforms the original ELMo on various sentence classification and language inference tasks.

==> tables/tbl6.tex <==
% {
% \begin{table}[t]
% \centering
% {
% \setlength\tabcolsep{1pt}
% \small
% \begin{tabular}{|l|l|l|}
% \hline
% \textbf{Sent. Pairs (Gold Standard Score)}  & \textbf{L2 Dist.} & \textbf{Score}  \\ \hline
% \begin{tabular}[c]{@{}l@{}}There is a cook preparing food.\\ A cook is making food. (5)\end{tabular} & \multicolumn{1}{c|}{1.1/\textbf{0.5}}       & \multicolumn{1}{c|}{3.7/\textbf{4.2}}    \\ \hline
% \begin{tabular}[c]{@{}l@{}}You are right on about the sample definition.\\You are on the right path. (0) \end{tabular}     & \multicolumn{1}{c|}{2.4/\textbf{1.5}}       & \multicolumn{1}{c|}{1.8/\textbf{1.3}}    \\ \hline
% \end{tabular}
% }
% \caption{Result of STS-Benchmark. L2 distance and predicted scores by vanilla ELMo, and those by ELMo-PCR trained on PAN (boldfaced). 
% }\label{tbl:sts}
% % BiSAE refers to BiDAF + Self Attention + ELMo.
% \end{table}
% }
{
\begin{table}[t]
\centering
\setlength\tabcolsep{2pt}
\small
\begin{tabular}{|l|c|c|} 
\hline
\textbf{Paraphrased contexts}& \textbf{L2} & \textbf{Cosine}  \\ \hline
\begin{tabular}[c]{@{}l@{}}How can I make \textbf{bigger} my arms? \\ How do I make my arms \textbf{bigger}?\end{tabular}  & 6.42 & 0.27 \\ \hline
\begin{tabular}[c]{@{}l@{}}Some people believe earth is \textbf{flat}. Why?\\ Why do people still believe in \textbf{flat} earth?\end{tabular} & 7.59 &   0.46           \\ \hline
\begin{tabular}[c]{@{}l@{}}It is a very \textbf{small} window. \\ I have a \textbf{large} suitcase. \end{tabular} & 5.44   &    0.26       \\ \hline
\end{tabular}
\caption{
% Paraphrase contexts where the same word (bold faced) have high embedding distances given by ELMo.
L2 and Cosine distance between embeddings of  boldfaced words. The distance between the shared word in the paraphrases are greater than such distance between
\emph{large} and \emph{small} in random contexts.
}\label{tbl:l2}. 
%\vspace{-2em}
\end{table}
}

